Foundational Question Generation for Video Question Answering via an Embedding-Integrated Approach

Conventional VQA approaches primarily rely on question-answer (Q&A) pairs to learn the spatio-temporal dynamics of video content. However, most existing annotations are event-centric, which restricts the model's ability to capture the comprehensive context of a scene. The lack of fundamental information such as object categories, spatial configurations, and descriptive visual attributes prevents the model from forming a complete understanding of the environment, ultimately limiting its generalization and reasoning capability. In this paper, we introduce Foundational Question Generation for Video Question Answering via an Embedding-Integrated Approach (FIQ), a framework designed to enhance the reasoning capability of VQA models by improving their foundational comprehension of video content. FIQ generates Q&A pairs from descriptive information extracted directly from videos, thereby enriching the dataset with core scene-level attributes. These generated pairs help the model develop a more holistic understanding of the video, leading to improved generalizability and reasoning performance. In addition, we propose a VQ-CAlign module that aligns task-specific question embeddings with corresponding visual features, preserving essential contextual cues and enhancing adaptability to downstream tasks. Experimental results on the SUTD-TrafficQA dataset demonstrate that FIQ achieves state-of-the-art performance, surpassing existing baseline approaches.

==> appendices.tex <==
\input{chapters/apppendix_pseudocode}

==> beginnings/acknowledgement.tex <==
% This research was supported by the Institute of Information \& Communications Technology Planning \& Evaluation (IITP) grant, funded by the Korea government (MSIT) (No. RS-2019-II190079 (Artificial Intelligence Graduate School Program (Korea University)), No. IITP-2025-RS-2024-00436857 (Information Technology Research Center (ITRC), and No. RS-2024-00457882 (AI Research Hub Project)).

This research was supported by the Institute of Information \& Communications Technology Planning \& Evaluation (IITP) grant, funded by the Korea government (MSIT) (No. RS-2019- II190079 (Artificial Intelligence Graduate School Program (Korea University)), and No. RS-2024-00457882 (AI Research Hub Project)).


% 이 패키지는 기존 \url{https://github.com/KUNPL/KUThesis}의 양식을 사용하여 고려대학교 학위논문 작성법이 요구하는 요소를 만족하도록 작성하였습니다. 석사/박사 영문논문 작성을 전제로 되도록 필요한 요소만을 남겨놓았으며, 대부분 주석을 통해 활용법을 안내하였으나, 기본적인 사용법을 아래에 설명드립니다.\par \bigskip
% *********** 사용법 ************* .\par \bigskip
% [박사과정의 경우] \par
% 1. 박사과정의 경우 "myThesisTemp.cls" 파일에서 line 20~23를 주석의 안내에 맞춰 수정한다. \par \bigskip
% [공통 사용법] \par 	
% 0. 컴파일러는 pdfLaTex 2014(legacy)로 설정하는 것을 권장합니다. \par
% 1. main.tex에서 논문제목, 이름, 지도교수명, 심사위원명단 등의 사항을 입력한다.\par
% 2. 초록, 서문, 감사의 글 등은 "beginnings" 폴더에 있는 각 파일에서 수정한다.\par
% 3. 본문의 경우 "chapters" 폴더에 있는 파일들을 참고해서 작성한다.\par
% 4. 본문 관련 tex파일을 추가하는 경우, "main.tex"파일에 \par 꼭 \verb|\addContents{chapters/~~~}|을 추가한다.\par
% 5. 참고문헌은 "library.bib" 파일에 저장한다.\par
% 6. 감사의 글, 서문, 사사 포함여부에 따라 "myThesisTemp.cls" 파일에서 line 277,279,281의 주석처리 여부를 결정한다.\par
% 7. 논문에 도식, 표 등의 포함여부에 따라 "myThesisTemp.cls" 파일에서 line 572,573의 주석처리 여부를 결정한다.\par \bigskip 

% [기타]\par
% 1) \verb|\bibitem|을 사용하여 Bibliography을 채우시는 분은 bibliography.tex를 따로 생성하여(이름은 바꿔도 상관없음) 그 파일에 인용 문헌을 적으시고 myThesisTemp.cls 파일 안의
% \verb|\bibliography{library.bib}| 대신 \par \bigskip
% \verb|\begin{thebibliography}{}|\par
% \verb|\input{bibliography.tex}|\par
% \verb|\end{thebibliography}| \par \bigskip
% 를 입력하시면 됩니다.\par \bigskip

% 2) Theorem, Lemma 등을 이용하고 싶으면 \par \bigskip

% \verb|\newtheorem{theorem}{Theorem}|\par
% \verb|\newtheorem{definition}{Definition}|\par
% \verb|\newtheorem{lemma}{Lemma}|\par
% \verb|\newtheorem{property}{Property}|\par \bigskip

% myThesisTemp.cls 파일 안의 Preamble 위에(아무데나 써도 상관은 없을테지만) 입력하면 됩니다.\par \bigskip

% 3) proof을 이용하고 싶으면 \verb|\RequirePackage|에 amsthm를 추가하면 됩니다.\par

% 4) appendix를 맨 마지막에 추가하려면 myThesisTemp.cls 파일 안의 bibliography 다음에 \par \bigskip

% \verb|\appendix| \par
% \verb|\input{appendices.tex}| \par
% \verb|\addevenpage|\par
% 를 입력하시면 됩니다.\par
% \par \bigskip
% 그 후 appendices.tex를 따로 생성하여 각 appendix를 \verb|\chapter|로 지정해주면 알파벳 형식 appendix가 나옵니다.\par


==> beginnings/dedicationpage.tex <==
감사의 글 예시 페이지입니다.

감사합니다.

==> beginnings/enabstract.tex <==
% Video question answering (VQA) is a multimodal task that when the video and the question related to the video are given as an input, generate the output as a text. Existing VQA methods primarily utilize question and answer (Q\&A) pairs to learn the spatio-temporal characteristics of video content. However, these annotations are typically eventcentric, which is not enough to capture the broader context of each video. The absence of essential details such as object types, spatial layouts, and descriptive attributes restricts the model to learning only a fragmented scene representation. This issue limits the model’s capacity for generalization and higher-level reasoning. In this paper, we propose a fundamental question generation with the integration of question embeddings for video question answering (FIQ), a novel approach designed to strengthen the reasoning ability of the model by enhancing the fundamental understanding of videos. FIQ generates Q\&A pairs based on descriptions extracted from videos, enriching the training data with fundamental scene information. Generated Q\&A pairs enable the model to understand the primary context, leading to enhanced generalizability and reasoning ability. Furthermore, we incorporate a VQ-CAlign module that assists task-specific question embeddings with visual features, ensuring that essential domain-specific details are preserved to increase the adaptability of downstream tasks. Experiments on SUTDTrafficQA demonstrate that our FIQ achieves state-of-the-art performance compared to existing baseline methods.

Conventional VQA approaches primarily rely on question-answer (Q\&A) pairs to learn the spatio-temporal dynamics of video content. However, most existing annotations are event-centric, which restricts the model’s ability to capture the comprehensive context of a scene. The lack of fundamental information such as object categories, spatial configurations, and descriptive visual attributes prevents the model from forming a complete understanding of the environment, ultimately limiting its generalization and reasoning capability. In this paper, we introduce Foundational Question Generation for Video Question Answering via an Embedding-Integrated Approach (FIQ), a framework designed to enhance the reasoning capability of VQA models by improving their foundational comprehension of video content. FIQ generates Q\&A pairs from descriptive information extracted directly from videos, thereby enriching the dataset with core scene-level attributes. These generated pairs help the model develop a more holistic understanding of the video, leading to improved generalizability and reasoning performance. In addition, we propose a VQ-CAlign module that aligns task-specific question embeddings with corresponding visual features, preserving essential contextual cues and enhancing adaptability to downstream tasks. Experimental results on the SUTD-TrafficQA dataset demonstrate that FIQ achieves state-of-the-art performance, surpassing existing baseline approaches.

\vspace*{\fill}
{\bf Keywords:} video question answering, spatio-temporal dynamics, question generation

% Video question answering (VQA) is a multimodal task in which a model receives both a video and a corresponding question as input and produces a textual answer as output. 

==> beginnings/krabstract.tex <==
기존의 VQA 접근법은 주로 질문–응답(Q\&A) 쌍을 활용하여 비디오 콘텐츠의 시공간적 특성을 학습하지만, 대부분의 주석이 사건 중심(event-centric)으로 구성되어 있어 장면의 전체적인 맥락을 충분히 포착하기 어렵습니다. 객체의 종류, 공간적 구성, 시각적 속성과 같은 기본적인 정보의 부재는 모델이 장면을 온전히 이해하는 것을 방해하며, 결과적으로 일반화 능력과 추론 성능을 제한합니다. 본 논문에서는 비디오의 근본적 이해를 향상시켜 모델의 추론 능력을 강화하기 위한 Foundational Question Generation for Video Question Answering via an Embedding-Integrated Approach(FIQ)를 제안합니다. 제안하는 FIQ는 비디오로부터 추출된 기술적 정보를 활용해 Q\&A 쌍을 생성함으로써, 데이터셋을 장면 수준의 핵심 속성으로 풍부하게 확장합니다. 이를 통해 모델은 비디오의 맥락을 보다 전체적으로 이해할 수 있게 되며, 결과적으로 일반화 및 추론 능력이 향상됩니다. 또한, VQ-CAlign 모듈을 도입하여 과제 특화 질문 임베딩과 시각적 특징을 정렬함으로써 필수적인 문맥 정보를 보존하고, 다양한 다운스트림 과제에 대한 적응력을 높입니다. SUTD-TrafficQA 데이터셋을 대상으로 한 실험 결과, 제안한 FIQ는 기존의 최신 기법들보다 우수한 성능을 달성하며, 비디오 이해 및 추론 성능의 향상을 입증하였습니다.

\vspace*{\fill}
{\bf 주제어:} 비디오 기반 질의응답, 시공간 정보, 질문 생성
% video question answering, , question generation
% 비디오 질문 응답 (Video Question Answering, VQA)은 주어진 비디오와 그에 대응하는 질문을 입력으로 받아 텍스트 형태의 답변을 생성하는 다중 모달(multimodal) 과제이다. 

==> beginnings/preface.tex <==
This dissertation is submitted for the degree of Master of Science in Artificial Intelligence at Korea University. This research was conducted under the supervision of Professor Seong-Whan Lee in the Department of Artificial Intelligence at Korea University. A portion of the study has been submitted for presentation at the 2025 IEEE International Conference on Systems, Man, and Cybernetics (SMC 2025). I served as the principal investigator for the projects, taking primary responsibility for conceptual development, data collection and analysis, and the preparation of the manuscript. This dissertation, or any work substantially similar to it, has not been submitted and is not under consideration for any other degree, diploma, or qualification at any other institution.
